Soft mechanical metamaterials with transformable topology protected by stress caching

Maxwell lattice metamaterials possess a rich phase space with distinct topological states featuring mechanically polarized edge behaviors and strongly asymmetric acoustic responses. Until now, demonstrations of non-trivial topological behaviors from Maxwell lattices have been limited to either monoliths with locked configurations or reconfigurable mechanical linkages. This work introduces a transformable topological mechanical metamaterial (TTMM) made from a shape memory polymer and based on a generalized kagome lattice. It is capable of reversibly exploring topologically distinct phases of the non-trivial phase space via a kinematic strategy that converts sparse mechanical inputs at free edge pairs into a biaxial, global transformation that switches its topological state. Thanks to the shape memory effect, all configurations are stable even in the absence of confinement or a continuous mechanical input. Topologically-protected mechanical behaviors, while robust against structural (with broken hinges) or conformational defects (up to ~55% mis-rotations), are shown to be vulnerable to the adverse effects of stored elastic energy from prior transformations (up to a ~70% reduction in edge stiffness ratios, depending on hinge width). Interestingly, we show that shape memory polymer's intrinsic phase transitions that modulate chain mobility can effectively shield a dynamic metamaterial's topological response (with a 100% recovery) from its own kinematic stress history, an effect we refer to as "stress caching".

==> Arxiv submission/jabbrv-master/INSTALL <==
===Basic Installation===
No installation is necessary, simply work in the same folder as the LaTeX style
file (jabbrv.sty), the language definition files (*.ldf) and the BibTeX style
files (*.bst).  Include the package by using \usepackage{jabbrv} in your LaTeX
preamble and enable the package functionality by setting the BibTeX
bibliography style to one of the following choices (depending on the desired
bibliography format):
	* jabbrv_abbrv
	* jabbrv_acm
	* jabbrv_alpha
	* jabbrv_ieeetr
	* jabbrv_plain
	* jabbrv_siam
	* jabbrv_unsrt

===Global Installation===
To attempt an automated global installation first open a terminal and change
the directory to the extracted jabbrv folder. Next, run the install script by
executing:
sudo ./install.sh

If the script cannot detect your local LaTeX installation folder, then you may
pass a custom install directory like so:
sudo ./install.sh /usr/local/share/texmf
Please note that the chosen folder must be part of the directory tree recognized
by your LaTeX installation, otherwise the package will note be properly detected.

===Using Other Styles===
If you wish to use a style outside of the base BibTeX package then you need to
modify that style to call jabbrv.  Start by copying the BibTeX style you wish
to use to your working folder (and rename it appropriately).  Next open the
style file and search for:
	"journal" output.check
This line is usually formatted like so (sometimes with an open bracket at
the beginning of the line):
	journal emphasis "journal" output.check
Replace this line (do not replace the open bracket if there is one) with:
	format.journal "journal" output.check
Then add the following code somewhere outside of the listed functions (above
the "article" function you're currently editing is fine):
	FUNCTION {format.journal}
	{
	  "{\em\JournalTitle{" journal * "}}" *
	}
Please note that if the line you replaced used some other formatting (we
started with an emphasized entry, corresponding to the "\em" command) then you
will need to change the formatting in the above function.  Once you have done
this step you should be all set, just follow the basic installation
instructions above.

===LyX Notes===
The preamble may be modified by choosing "Settings" from the "Documents" menu
and then selecting "LaTeX Preamble" from the menu on the left.


==> jabbrv-master/INSTALL <==
===Basic Installation===
No installation is necessary, simply work in the same folder as the LaTeX style
file (jabbrv.sty), the language definition files (*.ldf) and the BibTeX style
files (*.bst).  Include the package by using \usepackage{jabbrv} in your LaTeX
preamble and enable the package functionality by setting the BibTeX
bibliography style to one of the following choices (depending on the desired
bibliography format):
	* jabbrv_abbrv
	* jabbrv_acm
	* jabbrv_alpha
	* jabbrv_ieeetr
	* jabbrv_plain
	* jabbrv_siam
	* jabbrv_unsrt

===Global Installation===
To attempt an automated global installation first open a terminal and change
the directory to the extracted jabbrv folder. Next, run the install script by
executing:
sudo ./install.sh

If the script cannot detect your local LaTeX installation folder, then you may
pass a custom install directory like so:
sudo ./install.sh /usr/local/share/texmf
Please note that the chosen folder must be part of the directory tree recognized
by your LaTeX installation, otherwise the package will note be properly detected.

===Using Other Styles===
If you wish to use a style outside of the base BibTeX package then you need to
modify that style to call jabbrv.  Start by copying the BibTeX style you wish
to use to your working folder (and rename it appropriately).  Next open the
style file and search for:
	"journal" output.check
This line is usually formatted like so (sometimes with an open bracket at
the beginning of the line):
	journal emphasis "journal" output.check
Replace this line (do not replace the open bracket if there is one) with:
	format.journal "journal" output.check
Then add the following code somewhere outside of the listed functions (above
the "article" function you're currently editing is fine):
	FUNCTION {format.journal}
	{
	  "{\em\JournalTitle{" journal * "}}" *
	}
Please note that if the line you replaced used some other formatting (we
started with an emphasized entry, corresponding to the "\em" command) then you
will need to change the formatting in the above function.  Once you have done
this step you should be all set, just follow the basic installation
instructions above.

===LyX Notes===
The preamble may be modified by choosing "Settings" from the "Documents" menu
and then selecting "LaTeX Preamble" from the menu on the left.

